Distribution-Free Distribution Regression

`Distribution regression' refers to the situation where a response Y depends on a covariate P where P is a probability distribution. The model is Y=f(P) + mu where f is an unknown regression function and mu is a random error. Typically, we do not observe P directly, but rather, we observe a sample from P. In this paper we develop theory and methods for distribution-free versions of distribution regression. This means that we do not make distributional assumptions about the error term mu and covariate P. We prove that when the effective dimension is small enough (as measured by the doubling dimension), then the excess prediction risk converges to zero with a polynomial rate.

==> DFDR_ddrates.tex <==
 
\section{Rates for doubling dimension $d_0$}
\label{section::doublerate}



From theorem \ref{thm:upper.bound}, we have that 
 \begin{align*}
R(m) &\leq
\frac{1}{h}\bigg[
 C_1m\mathbb{E}(b)+C_2m\mathbb{E}\left(\frac{1}{n^{1/2} b^{k/2}}\right)\\
&\qquad  +\sum_{i=1}^m C_3\mathbb{E}(b_i) + C_4{\mathbb{E}\left(\frac{1}{n_i^{1/2} b_i^{k/2}}\right)}\bigg] +
C_5 h^\beta \\
&\qquad + C_6 \sqrt{\frac{1}{m h^{d_0}}}.
\end{align*}

Assuming for simplicity that $n=n_i$ and $b_i = b$ for all $i$,  we obtain
 \[
 R(m,n) \leq O \left( \frac{m}{h} \left[  \left(  b + \frac{1}{\sqrt{n b^k}} \right) + h^\beta + \frac{1}{\sqrt{m h^{d_0}}}\right] \right).
 \]
 
 Optimizing over $b$ yields
 \[
 R(m,n) = O \left( \frac{m}{hn^{1/(k+2)}} +
 h^{\beta} +\sqrt{\frac{1}{m h^{d_0}}}\right),
 \]
for usual choice of bandwidth $b = \Theta\left( n^{-\frac{1}{k+2}}\right)$.
 \todo[inline]{but notice the extra term $m$ now in the resulting expression for the risk...}
We now consider two cases. First, assume that the number of samples per distribution is very large compared to the number of distributions, i.e.
 \[
 n =  \Omega\left( m^{\frac{(3 \beta + d + 1) (k+2) }{2 \beta + d}}\right).
 \]
Then the term $ \frac{m}{hn^{1/(k+2)}} $ becomes negligible compared to $\sqrt{\frac{\log m}{m h^{d_0}}}$ and the optimal choice for $h$ is $h = \Theta \left( m^{- \frac{1}{2 \beta +d_0}}\right)$, leading to the rate
 \[
 R(m,n) = O \left( m^{-\frac{\beta}{2 \beta + d_0}} \right).
 \]
Thus, if the number of samples per distribution
$n$ is large, then the learning rate is limited by the number of labeled
observations $m$ and is in fact precisely the same as the
rate of learning a standard $\beta$-H\"{o}lder smooth regression function in
$d_0$ dimensions. That is, the the effect of not knowing the distributions
$P_1, \dots, P_m$ exactly and only having a finite sample from the distributions
is negligible.

 
 
The second case is more delicate, as it is no longer possible to analyze  the case of a large number  $m$ of distribution separately from $n$, and it appears instead necessary to sandwich the rate of growth of $m$. More precisely, assume that
\[
  \Omega \left(  n^{\frac{2 \beta + d_0}{(k+2)(3 \beta + d_0 + 1)}} \right) = m = O \left( n^{\frac{1}{k+2}} \right)
\]
 i.e.  the number of distributions is ``large" compared to the number of samples per distribution, in the sense that  $ \frac{m}{hn^{1/(k+2)}} $dominates $\sqrt{\frac{\log m}{m h^{d_0}}}$. However $m$ cannot be arbitrarily large now. Indeed,  the optimal choice for $h$ becomes
 \[
 h = \Theta \left( m^{\frac{1}{\beta+1}} n^{- \frac{1}{(\beta+1)(k+2)}} \right).
 \]
The reason for the upper constraint on $m$ shown above is now clear: it guarantees that $h$ vanishes as both $m$ and $n$ grow.  
  The corresponding rate is mixed in  $m$ and $n$:
 \[
 R(m,n) = O \left( m^{\frac{\beta}{\beta+1}} n^{- \frac{\beta}{(\beta+1)(k+2)}} \right).
 \]
 
 \todo[inline]{There is no dependence of $d_0$ now! double check this rates and comments}
 
 
 \todo[inline]{this is the old analysis of the rates which did not have the term $m$}
 
As a corollary, we have that
 \begin{equation}
R(m) \leq
\frac{1}{h}\left[
C_1 \mathbb{E}(b_i) + \sqrt{\mathbb{E}\left(\frac{C_2}{n_i b_i^k}\right)}\right] +
C_3 h^{\beta} + C_4 \sqrt{\frac{\log m}{m h^{d_0}}}.
\end{equation}

In the special case where $n_i = n$ and $b_i = b$ we have
\begin{equation}
R(m) \leq
\frac{1}{h}\left[
C_1 b + \sqrt{\left(\frac{C_2}{n b^k}\right)}\right] +
C_3 h^{\beta} + C_4 \sqrt{\frac{\log m}{m h^{d_0}}}.
\end{equation}

%AS ---------------%
Below $C$ may denote a different constant from line to line.

Optimizing over $b$ we get
\begin{equation}
R(m,n) = O\left(
\frac{1}{hn^{1/(k+2)}} +
C_3 h^{\beta} + C_4 \sqrt{\frac{\log m}{m h^{d_0}}}\right).
\end{equation}
for $b = Cn^{-1/(k+2)}$. %\left(\frac{C_2}{C_1^2n}\right)^{1/(k+2)}$.
If $$n = \Omega\left((m/\log m)^{((\beta+1)(k+2))/(2\beta+d_0)}\right),$$
we can choose $h = Cm^{-1/(2\beta+d_0)}$ and get
\begin{equation}
R(m,n) = O\left(
 m^{-\beta/(2\beta+d_0)}\right).
\end{equation}
This is reasonable because if the number of samples per distribution
$n$ is large, then the learning rate is limited by the number of labeled
observations $m$ and is in fact precisely the same as the
rate of learning a standard $\beta$-H\"{o}lder smooth regression function in
$d_0$ dimensions. That is, the the effect of not knowing the distributions
$P_1, \dots, P_m$ exactly and only having a finite sample from the distributions
is negligible.

On the other hand if the number of labeled observations are enough, specifically
$$(m/\log m)^{((\beta+1)(k+2))/(2\beta+d_0)} = \Omega(n),$$
we can choose $h = Cn^{-1/((\beta+1)(k+2))}$ and get
\begin{equation}
R(m,n) = O\left(
 n^{-\beta/((\beta+1)(k+2))}\right).
\end{equation}
In this case, the rate is limited by the number of samples per distribution $n$, as
expected. Notice that the rate gets worse as the dimensionality of each distribution
$k$ grows and as the smoothness $\beta$ of the regression function deteriorates.

While the rates seem reasonable, establishing optimality of the rates by demonstrating
matching lower bounds is an open question that we plan to investigate in future work.

 

==> DFDR_rates.tex <==
\section{Rates}
